AlphaMatch: Improving Consistency for Semi-supervised Learning with Alpha-divergence

Semi-supervised learning (SSL) is a key approach toward more data-efficient machine learning by jointly leverage both labeled and unlabeled data. We propose AlphaMatch, an efficient SSL method that leverages data augmentations, by efficiently enforcing the label consistency between the data points and the augmented data derived from them. Our key technical contribution lies on: 1) using alpha-divergence to prioritize the regularization on data with high confidence, achieving a similar effect as FixMatch but in a more flexible fashion, and 2) proposing an optimization-based, EM-like algorithm to enforce the consistency, which enjoys better convergence than iterative regularization procedures used in recent SSL methods such as FixMatch, UDA, and MixMatch. AlphaMatch is simple and easy to implement, and consistently outperforms prior arts on standard benchmarks, e.g. CIFAR-10, SVHN, CIFAR-100, STL-10. Specifically, we achieve 91.3% test accuracy on CIFAR-10 with just 4 labelled data per class, substantially improving over the previously best 88.7% accuracy achieved by FixMatch.

==> semi_supervised_learning _cvpr2021/tex/conclusion.tex <==
\section{Conclusion}
In this paper, 
we propose to use alpha-divergence and a new optimization-based framework to build a semi-supervised learning algorithm based on data augmentation.
The proposed AlphaMatch is simple yet powerful. %method. 
With only a few lines of extra code to implement alpha-divergence and the EM-like update,
it achieves the state-of-the-art performance on various benchmarks. 
%e.g. CIFAR-10, CIFAR-100, SVHN.

For future work, we will apply our algorithm to more practical tasks, e.g. 2D/3D segmentation, machine translation, object detection. 
% Second, 
By further extending and improving our framework, it is promising to push the frontier of ML with limited data to close the gap between few-shot learning and SSL.
Finally, we plan to extend our algorithm to unsupervised learning, out-of-distribution detection and other related topics.


==> semi_supervised_learning _cvpr2021/tex/experiment.tex <==
\section{Experiments}
%
%In this section, 
We test  AlphaMatch on a variety of standard SSL benchmarks (e.g. STL-10, CIFAR-10, CIFAR-100 and SVHN) and compare it with a number of state-of-the-art (SOTA) SSL baselines, including MixMatch \citep{berthelot2019mixmatch}, ReMixMatch \citep{berthelot2019remixmatch} and FixMatch \citep{sohn2020fixmatch}.
We show that AlphaMatch achieves the best performance in all benchmark settings evaluated.
% We show our method achieves significant improvements on all settings. 
% significantly improve on prior art baselines. 
% For all the experiments in the section, 

We use the code-base provided in FixMatch \citep{sohn2020fixmatch}\footnote{\url{https://github.com/google-research/fixmatch}} for implementation. 
Throughout our experiments, we simply set $\alpha=1.5$ and
$\beta=0.5$ without tuning; we found the default setting yields the best performance in almost all the cases. We provide comprehensive ablation studies on the impact of different choices of $\alpha$ and $\beta$ in section~\ref{sec:ablation}.


\subsection{STL-10}
We conduct experiments on the challenging SLT-10 dataset.
% , on which our method again shows clear advantage over existing methods.
SLT-10 is a realistic and challenging SSL dataset which 
contains 5,000 labeled images, and 
100,000 unlabeled, which are extracted from a similar but broader distribution of images than labelled data. 
The unlabelled data contains other types of animals (bears, rabbits, etc.) and vehicles (trains, buses, etc.) in addition to the ones in the labeled set.
The distribution shift between the labeled and unlabeled data casts a higher challenge for SSL algorithms, 
and requires us to learn models with stronger generalizability. 
%the unlabeled data are 
AlphaMatch again shows clear advantages over existing methods in this case. 

%\paragraph{Dataset and settings}The STL-10 \citep{coates2011analysis} dataset contains only 5,000 labeled images from 10 classes but upto 100,000 unlabeled images. The unlabeled images come from a similar but different distribution from the labeled data,thus forcing algorithms to learn underlying image statistics to achieve good performance and hence making it a more realistic challenging SSL test.

\paragraph{Settings}
%\red{Following }FixMatch \citep{sohn2020fixmatch}, 
We preprocess the data and split the labeled images into 5 folds with the same data partition as FixMatch \citep{sohn2020fixmatch}, with each partition containing 1,000 labels. 
Specifically, for each dataset, we use 4,000 labelled data and 100,000 unlabelled data to train and use the remained 1,000 labelled data to test.
Thus, a total of 5 models will be trained and evaluated. 
The final performance is averaged over these 5 individual runs. 

% We test SSL algorithms on five of the predefined folds of 1,000 labelled images each proposed by FixMatch. 
We use the Wide ResNet(WRN)-28-2 and WRN-16-8 model for our method and all the baselines.
% due to the computation resource limit. 
We compare AlphaMatch with $\pi$-model, unsupervised data augmentation (UDA), MixMatch, ReMixMatch and FixMatch. All baseline results are produced by 
exactly following the same training setting suggested in \citep{sohn2020fixmatch}.
For our method, we use the default setting of $\alpha=1.5$, $\beta=0.5$ and $n=1$.

\paragraph{Results}
We report the averaged accuracy of all 5 runs in Table~\ref{tab:stl}. 
AlphaMatch significantly outperforms all other baselines in this setting. 
In particular, for WRN-28-2, compared with FixMatch, we improve the accuracy from 89.28\% to 90.36\%.
Our performance is also about 1.9\% higher than ReMixMatch. 
For WRN-16-8, we also improve the baselines with a large margin.

\begin{table}[ht]
\begin{center} 
\begin{tabular}{l|cc}
\hline
Method & WRN-28-2 (\%) & WRN-16-8 (\%) \\
\hline
$\pi$-model & 71.39$\pm$1.21 & 74.92$\pm$1.18 \\
UDA & 86.57$\pm$1.06 & 89.14$\pm$0.73 \\
MixMatch & 85.19$\pm$1.24 & 87.52$\pm$0.79 \\
ReMixMatch & 88.42$\pm$0.78 & 91.07$\pm$0.84 \\
FixMatch & 89.28$\pm$0.63 & 91.35$\pm$0.67\\
\hline
AlphaMatch & \textbf{90.36$\pm$0.75} & \textbf{92.83$\pm$0.86}\\
\hline
\end{tabular}
\end{center}
\vspace{5pt}
\caption{ Testing accuracy on STL-10. All averaged over 5 different folds. Results on two different model architectures, WRN-28-2 and WRN-16-8 is reported.}
\label{tab:stl}
\end{table}



\begin{table*}[h]
    \centering
    % \footnotesize
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{lcccccc}
    \hline 
        \multirow{2}{*}{Method}& \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{SVHN} & \multicolumn{2}{c}{CIFAR-100} \\
         \cmidrule(l{3pt}r{3pt}){2-3}  \cmidrule(l{3pt}r{3pt}){4-5}
        \cmidrule(l{3pt}r{3pt}){6-7}
        & 40 labels & 250 labels  & 40 labels & 250 labels & 400 labels & 2500 labels\\
        % \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3}  \cmidrule(l{3pt}r{3pt}){4-5}
        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3}  \cmidrule(l{3pt}r{3pt}){4-5}
        \cmidrule(l{3pt}r{3pt}){6-7}
        Pseudo-Labeling & - & 50.22$\pm$0.43 & - & 79.79$\pm$1.09 & - & 42.62$\pm$0.46 \\ 
        UDA & 70.95$\pm$5.93 & 91.18$\pm$1.08 & 47.37$\pm$20.51 & 94.31$\pm$2.70 & 40.72$\pm$0.88 & 66.87$\pm$0.22 \\
        MixMatch & 52.46$\pm$11.50 &   88.95$\pm$0.86 & 57.45$\pm$14.53 & 96.02$\pm$0.23 & 33.39$\pm$1.32 & 60.06$\pm$0.37\\
        ReMixMatch & 80.90$\pm$9.64* & 94.56$\pm$0.05* & 96.64$\pm$0.30* & 97.08$\pm$0.48* & {55.72$\pm$2.06}* & {73.57$\pm$0.31}*\\
        FixMatch & 88.71$\pm$3.35 & 94.93$\pm$0.33 & 92.35$\pm$7.65 & 97.36$\pm$0.64 & 59.79$\pm$2.94* & 74.63$\pm$0.22*\\
        \cmidrule(l{3pt}r{3pt}){1-1} \cmidrule(l{3pt}r{3pt}){2-3}  \cmidrule(l{3pt}r{3pt}){4-5}
        \cmidrule(l{3pt}r{3pt}){6-7}
        % AlphaMatch & \bf{91.28$\pm$3.41} & \bf{95.01$\pm$0.28} & \bf{97.03$\pm$0.26} & \bf{97.56$\pm$0.32} & 51.57$\pm$2.90 & 71.96$\pm$0.41 \\
        AlphaMatch & \bf{91.35$\pm$3.38} & \bf{95.03$\pm$0.29} & \bf{97.03$\pm$0.26} & \bf{97.56$\pm$0.32} & \bf{61.26$\pm$3.13}* & \bf{74.98$\pm$0.27}* \\
        % + DA & - & - & - & - & \bf{61.26$\pm$3.13} & \bf{74.98$\pm$0.27} \\
        % \hline
        \hline 
    \end{tabular}

    \vspace{5pt}
    \caption{ 
    Testing accuracy (\%) of different methods on CIFAR-10, SVHN, and CIFAR-100. All averaged over 5 different  folds. The `*' indicates the results are achieved by combining the distribution alignment loss proposed in ReMixMatch \citep{berthelot2019remixmatch}. 
    }
    \label{tab:realistic_ssl}
\end{table*}
% \red{change Test accuracy and Test Accuracy to testing accuracy}


\subsection{CIFAR-10, SVHN and CIFAR-100}
\label{sec:ssl_cifar_ssl}
We then test AlphaMatch on three widely-used benchmark SSL datasets: 
CIFAR-10 \citep{krizhevsky2009learning}, 
SVHN \citep{netzer2011reading} 
and CIFAR-100. 
% We compare our method with several state-of-the-art semi-supervised learning 
% baselines on the standard CIFAR-10, SVHN and CIFAR-100 dataset. 
With only 4 labeled data per class, 
 we achieve  91.28\%$\pm$3.41\% accurcy on CIFAR-10, 97.03\%$\pm$0.26\% on SVHN, and 61.27\%$\pm$3.13\%  on  CIFAR-100, 
%testing accuracy  , SVHN and CIFAR-100, respectively, 
all of which yield 
significantly improvement over prior SSL results on this task.  
% the best performance on all three datasets,  

\paragraph{Settings} 
For a fair comparison, 
we proceed with minimum changes to the code provided by \citep{sohn2020fixmatch}.
% and keep all the hyper-parameters and settings as dafault.
Specifically, we use the same setting and random seeds 
as in FixMatch \citep{sohn2020fixmatch} to 
generate labeled and unlabeled data partitions. 
We use wide ResNet-28-2 \citep{zagoruyko2016wide} with 1.5M parameters as our prediction model,
and then train it using SGD with cosine learning rate decay for 1024 epochs. 
We use CTAugment \citep{berthelot2019remixmatch} for data augmentation as suggested in FixMatch \citep{sohn2020fixmatch}. 

We evaluate two SSL settings, which 
use 4 (resp. 25) labeled images per class, yielding 
40 (resp. 250) labeled images in CIFAR-10 and SVHN  and 
400 (resp. 2500) in  CIFAR-100. 
%and ii) 25 labeled images per class, yileding 
%250 labeled images in CIFAR-10 and SVHN 
%in which 4 or 25 images per class are labeled for supervision, respectively.  
%
%For the CIFAR-10 and SVHN dataset, the labeled set size is 40 and 250, respectively. 
%For CIFAR-100, the supervised data size is 400 and 2500. 
%
The remaining data in the training set is regarded as unlabelled data.
% we test 400 and 2500 labelled data setting.
For our method, we set $\alpha=1.5$ and $\beta=0.5$ by default 
and investigate the effect of $\alpha$ and $\beta$ in section \ref{sec:ablation}.
In order to maintain the similar training computation cost as FixMatch, 
We set the number of augmentation applied per image $n=1$ as default; the effect of $n$ is studied in section \ref{sec:ablation}. 
Following FixMatch, we combine AlphaMatch with an additional distribution alignment loss on  
CIFAR-100, which is proposed in ReMixMatch \citep{berthelot2019remixmatch}.
%Meanwhile, on CIFAR-100, we combine AlphaMatch with the distribution alignment loss, which is proposed by ReMixMatch \citep{berthelot2019remixmatch}. 

\vspace{-8pt}
\paragraph{Fully Supervised Baselines}
As a reference, 
we train fully-supervised baselines, i.e., training the models
with all the training labels available. 
The test accuracy is 96.14\%$\pm$0.03\%, 97.89\%$\pm$0.02\% and  79.17\%$\pm$0.01\% on CIFAR-10, SVHN and CIFAR-100, respectively. 

% to measure the highest
% test accuracy we could achieve. We 
\vspace{-8pt}
\paragraph{Results}
We report the test accuracy of all baselines \citep[][]{lee2013pseudo, xie2019uda, berthelot2019mixmatch, berthelot2019remixmatch, sohn2020fixmatch} along with AlphaMatch in Table \ref{tab:realistic_ssl}.
% in which the mean and variance \red{std?} of accuracy is computed on 5 different ``folds'' of random partitions.
All results are averaged over 5 random trials with different data partitions.
We can see that the models trained with AlphaMatch achieve the best performance in all the settings. 
% As we can see from Table~\ref{tab:realistic_ssl}, 
% our method outperforms FixMatch in all settings. 
The gain is especially significant
when the number of labeled data examples is limited (e.g. 4 labeled image per class).
In particular, compared with FixMatch, our method achieves  a 2.64\% improvement on  CIFAR-10 
and 4.58\% on SVHN for test accuracy. % on CIFAR-10 and , respectively. 
% On CIFAR-100, ReMixMatch \citep{berthelot2019remixmatch} yields the best performance in all baselines
% because of the distribution alignment loss it used.
% This loss adds a prior to the prediction on the augmented data.
On CIFAR-100, when combined with the distribution alignment loss as suggested in   \citep{berthelot2019remixmatch},  AlphaMatch yields the best performance, 
achieving
$61.26\%\pm3.13\%$ accuracy with 4 labels per class and 
and  $74.98\%\pm0.27\%$ with 25 labels per class.   
\subsection{Point Cloud Classification}
To further verify the effectiveness of our method, 
we conduct experiments for semi-supervised 3D point cloud classification.
We test a number of prior art SSL baselines and our
algorithm on ModelNet40 \citep{chang2015shapenet} using the SOTA Dynamic graph convolution neural network (DGCNN) \citep{wang2019dynamic}. 

\paragraph{Dataset}
ModelNet40 is the most widely adopted benchmark for point-cloud classification.  
It contains objects from 40 common categories.  There are 9840 objects in the training set and 2468 in the test set. 
% Objects are aligned to a common up and front direction.
In the experiment, we randomly select 100 objects for each category as labelled data and treat the other objects in the training set as unlabelled data.
It means, 
we use 4,000 labelled data and 5,420 unlabelled data during training and then evaluate the performance on the original test set.


\paragraph{Settings}
For all the baselines and our method, we use Gaussian blur $\mathcal{N}(0, 0.02)$ as weak augmentation, and using additional randomized jittering as strong augmentation.
For the DGCNN model, we use 2048 number of particles for each object and set the number of neighbours to 20.
We train the model with 2,00 epochs with SGD with cosing learning rate decay and 0.9 momentum.

\paragraph{Result}
We report the averaged accuracy of all 5 runs in Table~\ref{tab:pointcloud}. 
AlphaMatch significantly outperforms all other baselines in this setting. 
In particular, compared with FixMatch, we improve the accuracy from 86.5\% to 88.3\%.
Compared to other baselines, the proposed methods can also boost the performance by a large margin.
The result shows that our method  can also be applied to other settings except image classification.


\begin{table}[h]
\begin{center} 
\begin{tabular}{l|c}
\hline
Method & ModelNet40 Accuracy (\%) \\
\hline
$\pi$-model & 81.82$\pm$1.18 \\
UDA & 86.15$\pm$1.13  \\
MixMatch & 85.34$\pm$1.05  \\
ReMixMatch & 85.66$\pm$0.92  \\
FixMatch & 86.47$\pm$0.79 \\
\hline
AlphaMatch & \textbf{88.32$\pm$0.84} \\
\hline
\end{tabular}
\end{center}
\vspace{5pt}
\caption{ Testing accuracy on ModelNet40. All averaged over 5 different folds.}
\label{tab:pointcloud}
\end{table}

\subsection{Ablation Studies}
\label{sec:ablation}

\begin{figure*}[t]
\centering
\begin{tabular}{cc}
\raisebox{2.0em}{\rotatebox{90}{  Test Accuracy}}
\includegraphics[height=0.19\textwidth]{figures/ablation/beta_curve.pdf} &
\raisebox{2.0em}{\rotatebox{90}{ Test Accuracy}}
\includegraphics[height=0.19\textwidth]{figures/ablation/fig3.pdf} 
\raisebox{0.5em}{\includegraphics[width=0.145\textwidth]{figures/ablation/fig3_legend.pdf}}   \\
 ~~~(a) Training epoch ($\alpha=1.5$) & (b) choices of $\beta$ ~~~~~~~~~~~~~~~  \\
\end{tabular}
\vspace{5pt}
\caption{(b) The Learning curve of AlphaMatch on SVHN, when using  $\alpha=1.5$ and varying $\beta$.  The x-axis denotes the training epoch  and y-axis represents the test accuracy. 
% The labelled data includes 4 randomly picked mages per class.
The dashed line shows the result of FixMatch. 
% We follow all training settings in FixMatch.
(b) Testing accuracy of AlphaMatch with various $\alpha$ and $\beta$ on the SVHN dataset. 
All models are trained with 4 labeled examples per class. 
} 
\label{fig:ablation}
\end{figure*}
\vspace{5pt}

\begin{table*}[ht]
\begin{center} 
\begin{tabular}{c|cccc}
\hline 
$n$ augmented examples & 1 & 2 & 4 & 10\\
\hline
CIFAR-10 Accuracy (\%) & 91.35$\pm$3.38 & 91.48$\pm$3.41 & 91.63$\pm$3.12 & 91.59$\pm$3.08 \\
\hline
SVHN Accuracy (\%) & 97.03$\pm$0.26 & 97.07$\pm$0.19 & 97.18$\pm$0.23 & 97.18$\pm$0.21 \\
\hline 
\end{tabular}
\end{center}
\vspace{5pt}
\caption{ Comparison on testing accuracy for various $n$. All results are averaged over 5 random trials with the same settings as section \ref{sec:ssl_cifar_ssl}.
}
\label{tab:ablation_n}
\end{table*}

%\paragraph{A balance between $\alpha$ and $\beta$}
\paragraph{Impact of $\alpha$ and $\beta$} 
We follow all training settings as Section~\ref{sec:ssl_cifar_ssl}.
 All models are trained with 4 labeled examples per class.
% we create one dataset by randomly selecting 4 example per class on SVHN, and report the validation accuracy. 
On this dataset, FixMatch achieves $92.4\%$ test accuracy (see the dashed black line).
% Follow the settings in Figure \ref{fig:large_alpha},
In Figure~\ref{fig:ablation} (a), 
we fix $\alpha=1.5$ and study the impact of $\beta$. 
% As shown in Figure \ref{fig:ablation_beta},  
We find a smaller $\beta$ (e.g. $\beta=0.2$ or $0.5$) often yields more stabilized training; in the contrary, a larger $\beta$ (e.g. $\beta=0.8$) focuses less on clean (or weakly augmented) data and performs worse than small $\beta$ in general. 
% Our findings are consistent with our observation in Figure~\ref{fig:large_alpha}.
% See Section \ref{sec:ablation} for more details.

We plot in Figure~\ref{fig:ablation} (b) the testing accuracy of AlphaMatch with different $\alpha$ and $\beta $ %, and investigate their influence on the performance 
on SVHN dataset.  
As we can see from Figure~\ref{fig:ablation},
a larger $\alpha$ (e.g. $\alpha\ge 1.5$) and a smaller $\beta$ (e.g. $\beta\le 0.5$)
normally achieves better performance than FixMatch. 
% that $\alpha =1.5$,  $2.0$ or $3.0$ and $\beta=.2$; $\alpha = 1.5, \beta=0.5$ gives the best performance. 
%, that  
% and suffers from convergence issue, as we observe from Figure~\ref{fig:large_alpha}.
%the per
This is expected, as using alpha-divergence with large $\alpha$ values 
help propagate high confidence labels and a smaller $\beta$ helps to stabilize the training.
On the other hand, if $\alpha$ is too large, 
%and the stability 
the performance may diminish because numerical instability increases.

We observe that $\alpha=1.5$ and $\beta=0.5$ yields the best performance, 
achieving a good balance between consistency regularization and training stability. 
%in Figure~\ref{fig:ablation}).

\paragraph{Impact of the number of augmented examples $n$}
In our algorithm, $n$ controls on how many augmented examples is generated to approximate $\P_x$ (see Algorithm \ref{alg:main}). 
We can expect that $\{x_i'\}_{i=1}^n$ forms increasingly better approximation for $\P_x$ with a larger $n$. 
In this section, 
we perform an in-depth analysis on the effect of different $n$ values.
% In the experiments above, 
Intuitively, a smaller $n$ leads to better energy-efficiency
%on the other hand, 
while a larger $n$ is more computationally expensive but may yield more robust estimation hence produce better performance.

% we simply set $n = 1$ for best training efficiency. 
% let the computation cost of AlphaMatch and FixMatch the same.
% However, we can set $n$ larger to achieve better performance.
We test AlphaMatch on CIFAR-10 and SVHN, with the same settings as section~\ref{sec:ssl_cifar_ssl}. 
% \red{At each run, we randomly select 4 images per class as labeled training data.} \red{do not get what it means}  
% We conduct experiments on CIFAR-10 and SVHN with 4 labelled data per class,
% to display the impact of $n$ in \eqref{equ:gammat}. 
Table~\ref{tab:ablation_n} shows the performance of various $n$.
All results are averaged over 5 random trials.
We find $n=1$ often performs competitively and     
a larger $n$ (e.g. $n=4$, $n=10$) yields slightly improvements in general. 
However, a large $n$ can significantly increase the computation cost
since it increases the forward and backward time cost of the training model, and more critically, it requires a larger GPU memory cost.
Considering its huge time/memory cost and mild improvement, we recommend to use $n=1$ in practice.
% We find that a larger $n$ (e.g. $n=4$, $n=10$) often yields better performance compared 
% with a smaller $n$ (e.g. $n=1$, $n=2$). However, the gain is marginal. 
% Table \ref{tab:ablation_n} indicates that a larger $n$ (e.g. $n=4$, $n=10$) can have better performance than small $n$ (e.g. $n=1$, $n=2$).
% However, Table \ref{tab:ablation_n} also indicates  that larger $n$ can only sightly improve the results of the $n=1$ case
% with large additional computation cost.
% Hence, we do not refer to use large $n$ in practice.




==> semi_supervised_learning _cvpr2021/tex/introdution.tex <==
\section{Introduction}
%SSL
Semi-supervised learning (SSL) \citep{chapelle2009semi}
is a powerful paradigm for leveraging both labeled and unlabeled data jointly in machine learning (ML). 
%an simple yet efficient way to build machine learning systems with limited labelled data.
%
Effective SSL methods can help build accurate prediction out of very limited labeled data,
and can also boost state-of-the-art performance and robustness in typical supervised learning by leveraging extra unlabeled data  \citep[see e.g.,][]{xie2019self, kahn2020self, zhai2019adversarially}. 
Due to the high cost of collecting labels and 
the availability of a vast amount of unlabeled data, 
breakthroughs in SSL can dramatically 
%push the  
advance the application of ML in countless fields. 

Recently, data augmentation has been shown a powerful tool for developing  state-of-the-art SSL methods,  %in computer vision tasks, 
including unsupervised data augmentation (UDA) \citep{xie2019uda},  FixMatch \citep{sohn2020fixmatch}, MixMatch \citep{berthelot2019mixmatch}, ReMixMatch \citep{berthelot2019remixmatch} and $\Pi$-model \citep{rasmus2015pi}. 
All these methods are  based on 
%the key observation that the labels of the augmented images should be the same as the original images, and work by
the similar idea of enforcing the consistency between 
the label of a data point and that of its perturbed version generated by data augmentation. 
%the augmented data and that of the corresponding original data points. 
This encourages the learned models to be invariant under given data augmentation transforms, 
hence incorporating %informative invariance 
inherent
structures of the data into semi-supervised learning. 
%One popular class of SSL methods can be roughly viewed as first producing a label for each unlabeled data and then training the model to predict the label for each unlabelled data. 
% \emph{Pseudo-labeling} \citep{grandvalet2005semientropy} methods use the model’s class prediction as a label to train against. Recently, combining with data augmentation, a collection of efficient semi-supervised learning algorithms, including unsupervised data augmentation (UDA) \citep{xie2019uda},  FixMatch \citep{sohn2020fixmatch}, MixMatch \citep{berthelot2019mixmatch}, and ReMixMatch \citep{berthelot2019remixmatch}, have been developed enforcing the label consistency between the augmented images from the same images.
%\fi 

The performance of these algorithms can be critically influenced by 
%how the consistency is enforced and 
what matching objective and matching algorithm are used to enforce the consistency. 
%For example, although 
For the objective, 
UDA applies a KL divergence penalty to enforce the consistency uniformly on all the data points.
More recently, FixMatch shows that it is useful to 
focus on matching the consistency on the high confidence data points with a \emph{hard thresholding}  approach, 
%that the model is mostly confident with, 
by applying regularization only on data with  confidence higher than a threshold 
and use the hard label as the target.  %(rather than the probability, soft label) as the target.  
%Although works better, it is not ideal to ignore the data below the threshold, which can be still be useful. 
%enforces consistency between the
%However, this
%performing consistency updates on the 
%This is improved by 
%for the performance, 
%The different methods differ in the way how the consistency regularization is enforced. For example, UDA uses a typical KL divergence to enforce the consistency between augmented and original data.  FixMatch uses hard threshold and confidence-aware indicator function to focus more on high-confident data.Although it works better in practice, the divergence  would indeed have two optimal solution and therefore may make the optimization diverge in some cases.
%
In terms of the matching algorithm, 
most of the existing methods, including UDA and FixMatch, 
are based on a similar iterative regularization procedure that uses the label distribution predicted from the previous iteration as the target for the next step.
Although being simple and intuitive, 
a key problem is that this iterative procedure does not correspond to optimizing a fixed objective function, and hence may suffer from instability and non-convergence issues.  
%As a results, 
%many of these existing methods

This work proposes two key algorithmic advances to improve the objective and algorithm for consistency matching in SSL:  
 1) we propose to use alpha-divergence to measure the label consistency. 
%as the consistency measure for SSL.  
We show that, by using a large value of $\alpha$ in alpha-divergence, we can focus more on high confidence 
instances in a way 
similar to the hard-thresholded regularization of FixMatch, but in a more ``soft'' and flexible fashion.
%
2) We propose an optimization-based framework for consistency matching, which yields an  
EM-like algorithm 
with better convergence property than the commonly used iterative regularization procedures. %\qred{improve} 
%\red{This framework introduces an extra parameter to `smooth' the data augmentation prediction.}
By combining these two key techniques, 
our main algorithm \emph{AlphaMatch} 
yields better SSL with more effective and stable consistency regularization. 

Empirically, % results show that
we find that AlphaMatch consistently outperforms 
recently-proposed SSL methods such as FixMatch, ReMixMatch, MixMatch, and UDA  both in terms of  accuracy and data efficiency, 
on various benchmarks including  CIFAR-10, SVHN CIAFR-100, and STL-10.  
In particular, our method improves over the state-of-the-art method, FixMatch, across all the settings we tested. 
Our improvement is particularly significant  
when the labels are highly limited. 
%in very label-limited cases. % of only 4 labelled data per class.
For example, on CIFAR-10, 
we improve the 88.71\%$\pm$3.35\% accuracy of FixMatch to 91.35\%$\pm$3.38\% 
when only 4 labelled images per class are given.  
%\qred{more concrete?}
%In particular, when given only 4 labelled data per class, our method can significantly improve over FixMatch on [XXXX dataset?]. Under other settings, our method can also improve the results of FixMatch.
%It indicates that how to develop suitable divergence for the consistency regularization and how to smooth the data augmentation can be important topics for SSL.







==> semi_supervised_learning _cvpr2021/tex/method.tex <==
% \section{Methodology}
%\subsection{Objective and Update Mis-Match}
\section{Background: Semi-Supervision with Data Augmentation
}
\label{sec:bg}
%UDA and FixMatch}
 %Data augmentation has been shown to be a powerful tool for enabling efficient semi-supervised learning. 
%
We give a brief introduction to 
%the recent works for semi-superivsed image classification, 
unsupervised data augmentation (UDA) \citep{xie2019uda} and FixMatch \citep{sohn2020fixmatch}, which are mostly related to our work. 
Denote by $\D_s$ and $\D_u$ the labeled and unlabeled datasets, respectively.
% and $\D = \D_s \cup \D_u$ \red{we no longer need $\D$ since $\D_u$ was changed to $\D$?}.  
For a data point $x$ in $\D_u$, let $\P_x$ be 
a distribution that prescribes  
a random perturbation or augmentation transformation on $x$ that (with high probability) keeps the label of $x$ invariant,
such as rotation, shift, and cutout \citep{devries2017cutout}.
%unsupervised data augmentation in \cite{} suggested the following
For learning a prediction model $p_\theta(y|x)$, % with parameter $\theta$, 
UDA works by iteratively updating  the parameter $\theta$ via  
%unsupervised data augmentation (UDA) can be viewed as an iterative procedure of 
%xxx suggested to iteratively minimize the following objective function:  
\begin{align} 
%\theta_{t+1}=\arg\\
\begin{split} 
& \theta_{t+1}  \gets \argmin_{\theta} 
%\left\{L_{t}(\D; \theta) \overset{def}{=} 
\bigg\{ ~\L(\theta; ~\data_{s})  + 
\lambda  \Phi(\theta;\theta_{t},\D_u)~ \bigg\} ~~\text{with~~~~} \\
& \Phi(\theta;~\theta_{t}, \D_u) = \E_{x\sim \data_u, ~ x' \sim \P_x} \bigg [\KL(p_{\theta_t}(\cdot~|~x) ~\parallel~ p_\theta(\cdot ~|~ x')) \bigg] , 
%right\}, 
\end{split}
\label{eq:ssl-loss}
\end{align}
where $\theta_t$ denotes the value at the $t$-th iteration,  
$\L(\data_{s};~ \theta) $ is the typical supervised loss, e.g. the cross entropy loss, 
and  
$\KL(\cdot ~\pp~\cdot)$ denotes the Kullback–Leibler (KL) divergence. 
Here  $\Phi(\theta;\theta_{t},\D_u)$  
can be viewed as a consistency regularization %or self-supervision term 
that enforces the label distribution  of the augmented data $x'\sim \P_x$ to be similar to that of the original data $x$ (based on the parameter $\theta_t$ at the previous iteration); $\lambda$ is a regularization coefficient. 
% Intuitively, this can be viewed as 
% self-supervision on augmented data that uses the label distribution $p_{\theta_t}(\cdot|x)$ to guide the update of $p_{\theta}(\cdot|x')$. 
%The idea is that 
% and $\theta_0$ denotes the value of $\theta$ from the previous iterative, through which backpropagation is not applied. 
%

In practice, the optimization in \eqref{eq:ssl-loss}
can be approximated by applying one step of gradient descent initialized from $\theta_t$, yielding %UDA yields the following iterative procedure, 
\begin{align} 
%\!\!\!\!\!
\theta_{t+1} \gets 
\theta_{t} -  
\epsilon \nabla_{{\theta}}\bigg (\L(\theta; ~\data_{s})  + \lambda \Phi( \theta; ~\theta_{t}, ~ \D_u)
%\E_{x\sim \data, ~ x' \sim \P_x} \left [\KL (p_{\theta_{t}}(\cdot~|~x) ~||~ p_\theta(\cdot ~|~ x')) \right] 
\bigg) \bigg|_{\theta = \theta_{t}},  \label{equ:udagrad}
\end{align}
where $\epsilon$ is the step size. 
This procedure is closely related to  VAT \citep{miyato2015vat}, in which augmented data $x'$ is replaced by an adversarial example in a neighboring ball of $x$.
% , rather than random data augmentation.   %\red{introduce FixMatch, mention VAT?}
%

% \qred{Can we say some words of disadvantage of UDA w.r.t. FixMatch here? Check their paper to see what they said?}
FixMatch improves UDA with ideas similar to the classical \emph{pseudo-labeling} method \citep{grandvalet2005semientropy}.
FixMatch replaces the ``soft label'' $p_{\theta_t}(\cdot|x)$ 
%the idea by replacing the ``soft label'' $p_{\theta}(y|x)$ 
with the corresponding ``hard label''
$\hat y_{\theta_t}(x) = \argmax_y p_{\theta_t}(y~|~x)$ (a.k.a. pseudo-label), and  turns on the regularization only when   
the confidence of the pseudo-label, estimated by  $p_{\theta_t}(\hat y_{\theta_t}(x)~|~x)$, is sufficiently large: 
%by replacing KL divergence with 

\begin{align} 
\begin{split}
&\Phi(\theta; ~\theta_t, \D_u) := \E_{x\sim \D_u, x'\sim \P_x} \bigg [\ind\bigg(p_{\theta_t}(\hat y_{\theta_t}(x)~|~x) \geq \tau\bigg) \\ & \times \KL \bigg(\hat p_{\theta_{t}}(\cdot~|~x) ~\pp~ p_\theta(\cdot ~|~ x') \bigg) \bigg], \label{equ:fixmatch}
\end{split}
\end{align}

%where $\hat y_{\theta_t}(x) = \argmax_y p_{\theta_t}(y~|~x)$ (called the pseudo-label produced by model $p_{\theta_t}$) and 
where $\hat p_{\theta_{t}}(y~|~x) := \delta(y = \hat y_{\theta_t}(x))$ and $\ind(\cdot)$ is the indicator function and $\tau$ a threshold parameter (e.g., $\tau = 0.95$). 
This regularization has  two important effects:
1) it upweights the hard label $\hat y_{\theta_t}(x)$ while discarding all the other labels from the regularization, 
and 2) it skips the data points 
with low confidence (i.e., $p_{\theta_t}(\hat y_{\theta_t}(x)~|~x) < \tau$).
% \red{As shown in FixMatch \citep{sohn2020fixmatch}, 
% encouraging the model to propagate label confidence and stabilize the training objective, is important for semi-supervised learning.
% By using ``hard label'' and adding indicator function,
% FixMatch can be more stable than UDA when the model is trained for many iterations.}


\paragraph{Remark} 
Note that
the iterative procedure in \eqref{eq:ssl-loss}-\eqref{equ:udagrad}  
does not in general correspond  to optimizing a fixed objective function, 
and hence does not guarantee to converge theoretically and may suffer from non-convergence practically. 
For example, we empirically observe that the performance of UDA tends to degenerate significantly when trained for many iterations when few labelled data is given, and FixMatch is sensitive to the choice of threshold $\tau$. 
% \red{In practice, we does observe it has convergence issues.... Add something, but do not directly repeat what is said in the intro, maybe move the sentence on UDA in intro here.}
An alternative is to directly optimize the following objective function: 
% \red{$\Phi$ is the same definition as Eq 1. No need to repeat}
\begin{align} \label{equ:phithth}
\min_{\theta} \bigg\{ \L(\theta; ~ \data_s)  + \lambda \Phi(\theta; ~ \theta, ~ \data_u) \bigg\},
% , ~\text{with}~ \Phi(\theta; \theta, \D_u) = \E_{x\sim \data_u, ~ x' \sim \P_x} \bigg [\KL(p_{\theta}(\cdot~|~x) \pp p_\theta(\cdot ~|~ x')) \bigg], 
\end{align}
whose gradient descent yields 
\begin{align} 
\theta_{t+1} \gets 
\theta_{t} - 
\epsilon \nabla_{{\theta}}\bigg (\L(\theta; ~\data_{s})  + \lambda \Phi( \theta; ~\theta, ~ \D_u) 
%\E_{x\sim \data, ~ x' \sim \P_x} \left [\KL (p_{\theta_{t}}(\cdot~|~x) ~||~ p_\theta(\cdot ~|~ x')) \right] 
\bigg) \bigg|_{\theta = \theta_{t}}.  \label{equ:ggrad}
\end{align}
The difference with \eqref{equ:udagrad} is that the gradient of $\Phi(\theta; ~ \theta_t, \data_u)$ through $\theta_t$ 
 is detached and dropped in  \eqref{equ:udagrad}, 
while the gradient of $\Phi( \theta; ~\theta, ~ \D_u) $ in \eqref{equ:ggrad} needs to be taken for both $\theta$. In \citet{miyato2015vat, xie2019uda, sohn2020fixmatch} and all the related works, \eqref{equ:udagrad} is chosen over \eqref{equ:ggrad} for better empirical performance, likely because stopping the gradient encourages the information to pass from the clean data $x$ to the augmented data $x'$, but not the other way,  so that the supervised objective is less interfered by the consistency regularization than in the direction optimization approach \eqref{equ:ggrad}. 
A complete theoretical understanding of the benefit of stopping gradient is still an open question. %although the theoretical reason for fevering th%This is very similar to \eqref{equ:udagrad}, 

\iffalse
\dilin{do we need to introduce this?}
On the other hand, in the case when there is no data augmentation, that is, $\P_x(x) = \delta(x' = x)$, where $\delta$ is the delta measure, the iterative updates in \eqref{eq:ssl-loss} with KL divergence corresponds to minimizing the supervised loss $L(\theta; ~\data_s)$ with an entropic proximal point method and hence guarantees to converge. 
Also without data augmentation, FixMatch reduces to the classical self-training, which also corresponds to minimizing a fixed objective function. But this does not hold when the data augmentation is introduced. 
\fi

\begin{figure*}[h]
\centering
\setlength{\tabcolsep}{1pt}
% \begin{tabular}{c}
% FIXME
% % \raisebox{1em}{\rotatebox{90}{ Accuracy}}
% \includegraphics[height=0.35\textwidth]{figures/diagram.pdf} 
\includegraphics[height=0.32\textwidth]{figures/alpha_ssl.pdf} 
% \end{tabular}
\caption{
Diagram of our proposed semi-supervised learning algorithm. When augmentation, we use a hyper-parameter $\beta$ to control a mixture of strong and weak augmentation. When calculating the loss, we use a EM-style update. 1) Solving a closed-from solution of averaging logits with alpha divergence. 2) Using alpha divergence to construct a label-consistency loss. Images are from ImageNet \cite{deng2009imagenet}. 
}
\label{fig:diagram}
\end{figure*}

\section{Our Method}

% Despite the improvement, 
% the FixMatch regularization \eqref{equ:fixmatch}  
% can be sensitive to the threshold $\tau$, since using indicator function may make the objective diverge.
% % The use of hard label may also cause problem for real-world data.
% % For example, the unlabelled data is out-of-distribution or multi-class in real-world case, and therefore  the hidden is not discriminative.
%\red{todo..}W
We introduce our main method \emph{AlphaMatch} (see Algorithm~\ref{alg:main}),  
which consists of two key ideas: 
i) 
%Our first idea is to  
we leverage alpha-divergence to  enforce the label consistency  
between augmented and original data in SSL, which can benefit from focusing more on high confidence data  like FixMatch, 
but in a more smooth and flexible fashion (Section~\ref{sec:alpha});  
ii) we introduce 
a convergent 
EM-like algorithm based on an optimization-based framework to replace the iterative procedure in \eqref{eq:ssl-loss}-\eqref{equ:udagrad}, which allows us to enforce the label consistency much efficiently.  



\subsection{Matching with Alpha Divergence}
\label{sec:alpha}
%We propose to 
%\red{todo..}
%Our first idea is to  leverage alpha-divergence to  enforce the label consistency  between augmented and original data in SSL, which can benefit from focusing more on high confidence data  like FixMatch, but in a more smooth and stable fashion. %\citep{sohn2020fixmatch}, but would not diverge the optimization.
%
We propose to use alpha-divergence in 
SSL consistency matching. 
%to replace KL divergence 
Under the general framework of \eqref{eq:ssl-loss}, this amounts to replace the consistency regularization with 
\begin{align*} 
\Phi(\theta; ~\theta_t, \mathcal D_u) 
= \E_{x\sim \D_u, x'\sim \P_x} \bigg[D_\alpha(p_{\theta_t}(\cdot ~|~ x) \pp~ p_\theta(\cdot ~|~ x'))\bigg], 
\end{align*} 
%Recall that
where $D_\alpha(\cdot ~\pp~ \cdot)$ is the alpha divergence with  $\alpha\in (0,1) \cup (1,\infty)$, defined as: 
%
%
%
%
%
%
\begin{align*} 
\begin{split} 
& D_\alpha(p_{\theta_t}(\cdot|x)~||~p_\theta(\cdot|x'))
\\ & = \frac{1}{\alpha(\alpha-1)}\left (\E_{y\sim p_{\theta_t}(\cdot|x)} \left[ \rho_{D_\alpha}(y|x)\right]
%{p_\theta(y|x')^{1-\alpha}}
-1 \right), \\ &
~~\text{with}~~\rho_{D_\alpha}(y|x) := \bigg({\frac{p_{\theta_t}(y|x)}{p_{\theta}(y|x')} \bigg)^{{\alpha-1}}}.
%& = \frac{1}{\alpha(\alpha-1)}\left (\sum_{y} {p_{\theta_t}(y|x)^{\alpha}}{p_\theta(y|x')^{1-\alpha}}  -1 \right).
\end{split}
\end{align*}
It is well-known that $D_\alpha(\cdot||\cdot)$ reduces to KL divergence when $\alpha \to 0$ or $1$, as follows,
\begin{align*} 
& \lim_{\alpha \to 1} D_\alpha(p_{\theta_t}(\cdot|x)~\pp~p_\theta(\cdot|x'))  = \KL(p_{\theta_t}(\cdot|x)~\pp~p_\theta(\cdot|x')), \\
& \lim_{\alpha \to 0} D_\alpha(p_{\theta_t}(\cdot|x)~\pp~p_\theta(\cdot|x'))  = \KL(p_\theta(\cdot|x')~\pp~p_{\theta_t}(\cdot|x)).  
\end{align*}
% \red{it is about divergence not algorithm; but sjust remove this sentence: }Therefore, we obtain UDA without the \red{Training Signal Annealing (TSA) term } when $\alpha = 1$. 
In general, the value of $\alpha$ critically influences the result of the algorithm. 
%\red{todo...}
%plays a critical role in our algorithm. 
The regime of $\alpha > 1$ is  of particular interest for our purpose, %and can be seen to resemble 
because it allows us to achieve a FixMatch-like effect but in a ``soft way''. 
This is because when $\alpha$ is large, 
the power term %the power term
$\rho_{D_\alpha}(y|x)$ in $D_\alpha(\cdot||\cdot)$  tends to put a higher weight on the $(x,y)$ pairs with large values  of $p_{\theta_t}(y|x)$, and hence upweighting the importance 
the instances $x$ with high confidence as well as their dominating labels $y$. 
This is similar to what FixMatch attempts to achieve in \eqref{equ:fixmatch}, except that the regularization is enforced in a different and more ``soft'' 
fashion, so that the instances with lower confidence and the less dominant labels still contribute to the loss, except with a lower degree.  
%Therefore, it puts 
%which 

It is useful to get further insights by examining the gradient of $D_\alpha(\cdot||\cdot)$, which equals
%To see more, note that the gradient Alpha divergence is
% \begin{align} \!\!\!\!\!\!
% \nabla_\theta 
%  D_\alpha(p_{\theta_t}(\cdot|x)~||~p_\theta (\cdot|x'))  
% \propto \E_{y\sim p_{\theta_t}(\cdot | x)}  \bigg[\blue{\rho_{D_\alpha}(y|x)} \nabla_{\theta} \log p_\theta (y|x') \bigg], &&
% \rho_{D_\alpha}(y|x) = \left(\frac{p_{\theta_t}(y|x)}{p_\theta(y|x')}\right)^{\alpha-1}
% \label{equ:alpahgrad}
% \end{align}

\begin{align}
\begin{split}
\!\!\!\!
& \nabla_\theta 
 D_\alpha(p_{\theta_t}(\cdot|x)~\pp~p_\theta (\cdot|x'))  
\\ & =-\frac{1}{\alpha}\E_{y\sim p_{\theta_t}(\cdot | x)}  \bigg[\blue{\rho_{D_\alpha}(y|x)} \nabla_{\theta} \log p_\theta (y|x') \bigg]. %&&
%\rho_{D_\alpha}(y|x)=\left(\frac{p_{\theta_t}(y|x)}{p_\theta(y|x')}\right)^{\alpha-1}.
\label{equ:alpahgrad}
\end{split}
\end{align}
%where . 
When $\alpha=1$ (corresponding to UDA),  we have $\rho_{D_\alpha}(y|x) = 1$.  
%In comparison, 
The gradient of FixMatch is also similar but with $\rho_{D_\alpha}(y|x)$ replaced by 
\begin{align}
\begin{split}
& \rho_{\mathrm{FixMatch}} (y|x) = \\ 
& ~~~~\ind\Big(\max_{y'} p_{\theta_t}(y'|x) \geq \tau  \&y ~= \arg\max_{y'}(p_{\theta_t} (y'|x))  \Big).
\end{split}
\end{align}
We can again see that both $\rho_{D_\alpha}(y|x)$ and $\rho_{\mathrm{FixMatch}}(y|x)$ favor the  data and label $(x,y)$ with high  confidence   $p_{\theta_t}(y|x)$, but 
$\rho_{\mathrm{FixMatch}}(y|x)$ does it in a more aggressive fashion. 
In addition, note that $\rho_{D_\alpha}(y|x)$ depends on both $p_{\theta_t}(y|x)$ and $p_{\theta}(y|x)$, while $\rho_{\mathrm{FixMatch}}(y|x)$ only depends on $p_{\theta_t}(y|x)$. 

\paragraph{Remark}
% Alpha divergence because it is more natural fit for our purpose.
Alpha divergence provides a general framework for distribution matching. 
It's more flexible compared to other divergences, e.g., Jensen–Shannon divergence. By choosing different values of $\alpha$, our alpha divergence generalizes a number of well-known SSL approaches, including UDA ($\alpha=1$) and FixMatch ($\alpha\rightarrow \infty$). 
Furthermore, note that alpha divergence is proportional to the $\alpha$-th moment of density 
ratio $p(\cdot|x)/p(\cdot|x')$ ($x$ clean image and $x'$ augmented image). 
Therefore, when $\alpha$ is large and positive, large $p(\cdot|x)/p(\cdot|x')$ ratio is strongly penalized, preventing the case of $p(\cdot|x') \ll p(\cdot|x)$. 
This offers a natural and flexible way to propagate high confidence label on $x$ to low-confidence examples $x'$. 

\subsection{An EM-like Optimization Framework for Label Matching}

\begin{figure} %{r}{0.4\textwidth}
% \vspace{-5pt}
\centering
\begin{tabular}{c}
\raisebox{3.0em}{\rotatebox{90}{\large Test Accuracy}}
\includegraphics[height=0.26\textwidth]{figures/ablation/alpha_curve.pdf} \\
\large{~~~~Training epoch} \\
\end{tabular}
\caption{The learning curve of update Eqn  \eqref{equ:udagrad} with alpha-divergence  with different $\alpha$ 
  on SVHN. 
  %where we randomly pick up 4 image per class as labelled data, and regard the others in training set as unlabelled data. 
  The x-axis denotes the training epoch y-axis is the test accuracy. 
  The labelled data includes 4 randomly picked mages per class. 
  The dashed line shows the result of FixMatch. 
  We follow all training settings in FixMatch.
}
\label{fig:large_alpha}
\end{figure}

%The section above advocates to use 
Despite the attractive property of alpha-divergence, 
% with large $\alpha$. %However,% 
we observe that directly incorporating alpha-divergence 
%with the 
into the iterative update in \eqref{equ:udagrad} like UDA and FixMatch 
%
tends to cause instability in convergence when $\alpha$ is large, 
which is the regime of main interest. 
We illustrate this with an experiment on SVHN shown in Figure~\ref{fig:large_alpha}, 
which shows that using large $\alpha$ (e.g., $\alpha = 1.5$)
can potentially obtain better results than smaller $\alpha$ 
%better performance, 
but is much more unstable during training and may eventually diverge to worse results (note that the case of $\alpha = 1$ (blue curve) is UDA). 
This is because the iterative update in \eqref{eq:ssl-loss} does not  correspond to optimizing a well-defined objective and does not guarantee to converge theoretically.

%outperform the case with 
%small $\alpha$. 
%% for an illustration. 
%It displays that, 
% smaller $\alpha$ (e.g. $\alpha$ = 0.5) comes to stable training.
%larger $\alpha$ (e.g. $\alpha$ = 1.5) can perform better than small $\alpha$ during the training, but the training process is very unstable and thus finally leads to a worse result.
%\red{need refine this section; the part on figure 1 should be shortened } 
% even with very small step size.  
%\qred{However, when $\alpha $ is large, it suffer from convergence problem. }  \qred{$\beta$ helps adjust convergence.}

% \qred{TODO: remove $\P_x^\beta$? No need to introduce it?}

To address this problem, 
we provide an optimization-based  framework for consistency regularization, 
%that incorporate more flexible alpha divergence for  
which yields an EM-like algorithm when solved with a coordinate descent procedure.  
Our method enjoys better convergence and allows us to achieve better performance than directly combining alpha-divergence with \eqref{equ:udagrad}.  
%
%Consider the following loss
Our loss function is %defined as follows: 
\begin{align} 
\min_{\theta} \bigg\{ \L(\data_s;~ \theta) + \lambda  
%\E_{x\sim \data} \left [ D_{\alpha,\beta} (\gamma(\cdot~|~x) ~||~ p_\theta(\cdot ~|~x')) \right )\right]
\E_{x\sim \D_u}\bigg[
\min_{\gamma(\cdot~|~x)} 
\Psi_{\alpha,\beta}(\theta, \gamma, x)\bigg] \bigg\}, 
%\sum_{k} 
\label{equ:beta_obj}
\end{align}
where $\Psi_{\alpha,\beta}(\theta, x)$ is a consistency regularization on $x$ that we define as  
\begin{align} 
\begin{split} 
& \Psi_{\alpha,\beta}(\theta, \gamma, x) 
= 
(1-\beta ) D_\alpha (\gamma(\cdot~|~x) ~||~ p_\theta(\cdot ~|~x)) \\ & + \beta \E_{x'\sim \P_x}\left [ D_\alpha (\gamma(\cdot~|~x) ~||~ p_\theta(\cdot ~|~x')) \right]   \\
& =  
\E_{x'\sim \P_x^\beta}\left [D_\alpha (\gamma(\cdot~|~x) ~||~ p_\theta(\cdot ~|~x')) \right], 
\end{split}
\label{equ:beta_consistency}
\end{align}

where $\P_x^\beta(x') \overset{\mathrm{def}}{=} (1-\beta) \delta(x'= x) + \beta \P_x(x')$ is a mixture of the random perturbation $\P_x$ and the original data $x$  and $\beta \in [0,1]$ %that is, 
%$$\P_x^\beta(x') \overset{def}{=} \beta \delta(x'= x) + (1-\beta) \P_x(x'),$$
%$\beta$ 
is  the ratio between the augmented and original data in $\P_x^\beta$. 
Here $\gamma(\cdot~|~x)$ is an auxiliary variable 
optimized in the space of all distributions. It is 
introduced to serves as a bridge for comparing $p_\theta(\cdot | x)$ and $p_\theta(\cdot | x')$, without having $\theta$ appearing on sides of the divergence like $\Phi(\theta; \theta, \mathcal D)$ in \eqref{equ:phithth}. 
When $\beta = 0.5$, the regularization in \eqref{equ:beta_obj} 
  is a symmetrized version of alpha-divergence that generalizes Jensen-Shannon divergence. 

We optimize our objective function in \eqref{equ:beta_obj} by alterenaively optimizing $\theta$ and $\gamma$: 
%with a coordinate descent approach that optimizes $\theta$ and $\gamma$ alternatively. 
% Our method alternates between the following two steps: 

\paragraph{Updating $\gamma$}
With  $\theta = \theta_{t}$ fixed,  we update $\gamma(\cdot|x)$ for each $x$: 
%For each $x$, update $\gamma$ with : 
\begin{align}
{\gamma_{t}}(\cdot ~|~ x) \gets \argmin_{\gamma(\cdot|x)} 
 \E_{x' \sim \P_x^\beta} \Big [D_\alpha (\gamma(\cdot~|~x) ~\pp~ p_{\theta_{t}}(\cdot ~|~ x'))  \Big]. 
 \label{equ:update_gamma}
 \end{align}

\paragraph{Updating $\theta$} 
With $\gamma = \gamma_{t}$ fixed,  
we update $\theta$ %with fixed $\gamma = \gamma_{t}$
by performing gradient descent on 
\begin{align}
 {\theta_{t+1} }
 \gets  \argmin_{\theta} 
 L(\data_{s};~ \theta)  + 
 \lambda \E_{x\sim \D_u} \big [
%\min_{\gamma(\cdot~|~x)} 
\Psi_{\alpha,\beta}(\theta, \gamma, x)\big]. 
 %\lambda \E_{x\sim \data, ~ x' \sim \P_x^\beta} \left [D_\alpha (\gamma_{t}(\cdot~|~x) ~||~ p_\theta(\cdot ~|~ x')) \right]. 
%{\theta_{t+1} }\gets \theta_t - \epsilon \Delta(\theta_t; \D_s, \D_u), && \Delta(\theta_t; \D_s, \D_u) = \nabla_{\theta}\Big(\L(\data_{s};~ \theta)  + \lambda \E_{x\sim \D_u}[ \Psi_{\alpha,\beta}(\theta, \gamma_t, x)] 
%D_\alpha (\gamma_{t}(\cdot ~|~ x) ~\pp~ p_\theta(\cdot ~|~ x))] \Big)\bigg|_{\theta=\theta_t}, 
\label{equ:update_theta}
\end{align}
% \red{this can go into algorithm box;} \dilin{leave it here? otherwise the algorihtm box would be huge.} 
% \begin{align}
% %\E_{x'\sim \P_x^\beta}\bigg[D_\alpha (\gamma_{t+1}(\cdot ~|~ x) 
% \Psi_{\alpha,\beta}(\theta, \gamma_t, x)  
% %~\pp~ p_\theta(\cdot ~|~ x))\bigg] 
% \approx (1-\beta )
% D_\alpha (\gamma_{t}(\cdot ~|~x) ~\parallel~ p_\theta(\cdot ~|~x) )  + \frac{\beta}{n} \sum_{i=1}^n \Big [ D_\alpha (\gamma_{t}(\cdot ~|~x) ~\parallel~ p_\theta(\cdot ~|~x_i'))   \Big ].
% \label{equ:empirical_update_theta}
% \end{align}
 Critically, for alpha-divergence, 
 the optimal $\gamma_{t}$ in Eqn~\eqref{equ:update_gamma} 
 equals a simple powered expectation of $p_{\theta_{t}}(\cdot | x')$ as $x'\sim \P_x^\beta$, 
%has a simple closed form solution 
%For Alpha divergence, we have a closed form solution: 
\begin{align} 
\begin{split} 
\gamma_{t}&(\cdot ~|~x)   
\propto \left  (\E_{x'\sim  \P_x^\beta}\left [ p_{\theta_{t}}(\cdot~|~x')^{1 - \alpha}\right]\right )^{\frac{1}{1-\alpha}} =\\
&\bigg(  (1-\beta) p_{\theta_{t}} (\cdot~|~x)^{1-\alpha} +  \beta\E_{x'\sim \P_x}\left [ p_{\theta_{t}}(\cdot~|~x')^{1-\alpha}\right]\bigg )^{\frac{1}{1-\alpha}}.  \\
\end{split}
\label{equ:gammat}
\end{align}
% where the expectation on $\P_x$ is approximated with a set of $n$ augmented examples.
%\red{stopped here}

\begin{proof}
% Solving Eqn~\eqref{equ:update_gamma} could be viewed as minimizing an objective as follows, 
% that yields the minimum alpha divergence 
% to a set of distributions $\{p_i\}$. 
% $$
% \min_{\gamma } \sum_{i} w_i [D_\alpha(\gamma ~||~p_i) ], 
% $$
% = 
% \sum_i w_i \bigg(\int \frac{\gamma^\alpha}{p_i^{\alpha-1}}-1 \bigg). 
% $$ %yields that 
% We have 
% $$
% \gamma \propto  
% \left  (\sum_i w_i p_{i}^{1-\alpha}\right )^{\frac{1}{1- \alpha}}.
% $$
% Solving Eqn~\eqref{equ:update_gamma} could be viewed as finding the optimal $\gamma(\cdot\mid x)$ that minimizes a weighted alpha divergence to a set of distributions $p_{\theta_t}(\cdot\mid x')$ with $x'\sim \P_x^\beta$. 
Eqn~\eqref{equ:update_gamma} could be viewed as a general optimization of form:
$$
\min_{\gamma } \sum_{i} w_i [D_\alpha(\gamma ~||~p_i) ],
$$
where $w_i$ denotes the importance score for each distribution $p_i$.
With simple calculations, we have, 
\begin{align*}
&\sum_{i} w_i [D_\alpha(\gamma ~||~p_i) ]  = \sum_i w_i \sum_x \frac{\gamma^\alpha(x)}{p_i^{\alpha-1}(x)} \\
&  = \sum_x \sum_i w_i p_i^{1-\alpha} (x) \gamma^\alpha(x),  \\
&= \sum_x \bar{p}^{1-\alpha}(x) \gamma^\alpha(x), \text{with}~ \bar{p}(x) = \bigg(\sum_i w_i p_i^{1-\alpha}(x)\bigg)^{\frac{1}{1-\alpha}} \\ 
&= D_\alpha(\gamma || z \bar{p}), 
\end{align*}
where $z$ is the normalization constant. Therefore, we have
$\gamma^* \propto \bar{p}$.
\end{proof}

This formulation reduces to the typical averaging when $\alpha \to 0$, and 
the reduces to geometric mean when $\alpha \to 1$. 
On the other hand, 
when $\alpha \geq 1$, 
the regime of our interest, 
 $\gamma_{t}(\cdot | x)$ becomes a (powered) harmonic mean of $p_{\theta_{t}}(\cdot | x')$ when $x'\sim \P_x^\beta$. % and %$\gamma_{t+1}(\cdot | x)$ 
 %tends to be large only if $p_{\theta_{t+1}}(\cdot | x')$ is large for all $x'$. 
 %This 
 %can be seen by considering 
Consider the limit $\alpha \to+\infty$, in which case we have $\gamma_{t}(y | x) \approx \mathrm{ess}\inf_{x'\sim \P_x^\beta} p_{\theta_{t}}(y ~|~ x')$, 
which suggests that $\gamma_{t}(y | x)$ is large only when $p_{\theta_{t}}(y ~|~ x')$ are large for both the original data $x'=x$ and  all the augmented data $x'\sim \P_x$.  
This is again consistent with the idea of emphasizing 
high confidence instances. 
% %Overall, when $\alpha$ is large, the significance of large $\gamma(\cdot~|~x)$ is emphasized when matching $p$, and the significance of small $p$ is emphasized when calculating $\gamma$. The idea is that $\gamma$ should be determined by the most uncertainty (smallest) part of $p$, while $p$ should be determined by the most confident (largest) part of $\gamma$.  And this achieved by $\alpha \geq 0$. 

% In practice, we approximate $\E_{x' \sim \P_x}[\cdot]$ in \eqref{equ:gammat}
% with the same samples $\{x_i'\}_{i=1}^n$ generated in \eqref{equ:empirical_update_theta} for better training efficiency.
% yielding 
% \begin{align}
% \gamma_{t+1}(\cdot~|~x) \approx \bigg(  (1-\beta) \times p_{\theta_{t}} (\cdot~|~x)^{1-\alpha} +    \frac{\beta}{n} \times \sum_{i=1}^n  \bigg [ p_{\theta_{t}}(\cdot~|~x_i')^{1-\alpha}\bigg]\bigg )^{\frac{1}{1-\alpha}}.
% \label{equ:empirical_update_gamma}
% \end{align}
% with an additional hyper-parameter $n$, which denotes the number of samples. 
% See Algorithm \ref{alg:main} for details.
% We can expect that $\{x_i'\}_{i=1}^n$ forms increasingly better approximation for $\P_x$ with a larger $n$.  

%where $\epsilon$ is the step size. Empirically, 
%In practice, we approximate $\E_{x'\sim \P_x}[\cdot]$ in \eqref{equ:beta_consistency} and \eqref{equ:gammat} 
%(see Eqn.~\ref{equ:beta_consistency})by drawing a number of $n$ random samples $\{x_i'\}_{i=1}^n$ from $\P_x$.See Algorithm~\ref{alg:main} for details. 

\paragraph{Our method}
%\dilin{rephrase the sentence in intro a little:
Combining these two updates yields a simple and practical algorithm shown in Algorithm~\ref{alg:main},
in which we apply one-step of mini-batch gradient descent to update $\theta$ at each iteration and  approximate $\E_{x'\sim \P_x}[\cdot]$ in \eqref{equ:beta_consistency} and \eqref{equ:gammat} 
%(see Eqn.~\ref{equ:beta_consistency})
by drawing a number of $n$ random samples $\{x_i'\}_{i=1}^n$ from $\P_x$ for practical efficiency.  

Our method converges theoretically because it is a coordinate descent by design. 
It is similar in style to expectation maximization (EM), 
especially  the $\alpha$-EM \citep[e.g.,][]{matsuyama2003alpha} which uses alpha-divergence in EM. However, our method is designed from an optimization perspective for enforcing the label consistency on augmented data, rather than a generative modeling perspective underlying EM.  
%
%where $\epsilon$ is the step size. 
Empirically, we approximate $\E_{x'\sim \P_x}[\cdot]$ (see Eqn.~\ref{equ:beta_consistency}) by drawing a number of $n$ random samples $\{x_i'\}_{i=1}^n$ from $\P_x$.
See Algorithm~\ref{alg:main} for details. 

% \begin{algorithm*}[t]
% \caption{AlphaMatch: Improving Consistency for SSL with Alpha-divergence}
% \label{alg:main}
% \begin{algorithmic}[1]
% \STATE {\bf Input:} labeled data $\D_s$; unlabeled data $\D_u$; regularization coefficient $\lambda$;  alpha-divergence hyper-parameters $\alpha$ and $\beta$; 
% number of augmentation samples $n$;  initial model parameter $\theta_0$. 
% % \STATE {\bf Goal:} Find the best model parameter $\theta$ 
% % \STATE Initialize $\theta_0$
% \FOR{iteration $t$}
%     \STATE Randomly sample a labeled batch $B_s$ from $\D_s$ and an unlabeled batch 
%     $B_u$ from $\D_u$.  
%     \STATE \emph{Fix} $\theta = \theta_{t}$, \emph{update} $\gamma_{t+1}(\cdot|x)$ for each $x$ in $B_u$ according to~\eqref{equ:empirical_update_gamma} with $n$ augmented samples.
%      \STATE \emph{Fix} $\gamma=\gamma_{t+1}$, \emph{update} $\theta_{t+1} \leftarrow \theta_t - \epsilon \Delta(\theta; B_s, B_u)$ according to~\eqref{equ:update_theta}, where $\epsilon$ is the step size.
% %     \FOR{each $x$ in $B_u$}
% %     \STATE Apply strong data augmentation $n$ times, yielding augemted examples $\{x_i'\}_{i=1}^n$
% %     \STATE Estimate $\gamma_{t+1}^*$ using according to Eqn~\ref{equ:gammat}
% %      \STATE  Measure consistency loss for each $x$ using Eqn.~\ref{equ:beta_consistency}
% %      $$
% %      \Psi_\beta(\theta, x) = (1-\beta )
% % D_\alpha \bigg(\gamma_{t+1}^*(\cdot ~|~x) ~\parallel~ p_\theta(\cdot ~|~x)\bigg)  + \frac{\beta}{n} \sum_{i=1}^n \bigg [ D_\alpha (\gamma_{t+1}^*(\cdot ~|~x) ~\parallel~ p_\theta(\cdot ~|~x_i'))   \bigg ]
% %      $$
% %      \ENDFOR
% %      \STATE  Update $\theta_{t+1} \leftarrow \theta_t - \epsilon \Delta \theta$, with $\epsilon$ a step size, and 
% %      $$
% %      \Delta \theta = \theta_{t+1} \leftarrow \theta_t - \epsilon \nabla_{\theta}\bigg(\L(B_{s};~ \theta)  + \frac{\lambda }{|B_u|} \sum_{x\sim B_u} \bigg[\Psi_\beta(\theta, x)\bigg ]\bigg) \bigg|_{\theta=\theta_t} 
% %      $$
     
% %     % \STATE Update $\theta$ with fixed $\gamma$ with \eqref{equ:update_theta}
% %     % $$
% %     % \theta_{t+1} \leftarrow \theta_t - \nabla_\theta  \left [ \L(B_s; \theta) ~+~ \lambda \E_{x\sim B_u, ~ x' \sim \P_x^\beta} \left [D_\alpha (\gamma^*(\cdot~|~x) ~||~ p_\theta(\cdot ~|~ x')) \right]  \right ].
% %     % $$
% %     % with $L(\cdot)$ as the supervised loss (e.g. cross entropy). 
% \ENDFOR
% \end{algorithmic}
% \end{algorithm*}

\begin{algorithm*}[t]
\caption{AlphaMatch: Improving Consistency for SSL with Alpha-divergence}
\label{alg:main}
\begin{algorithmic}[1]
\STATE {\bf Input:} labeled data $\D_s$; unlabeled data $\D_u$; regularization coefficient $\lambda$;  alpha-divergence hyper-parameters $\alpha$ and $\beta$; 
number of augmentation samples $n$;  initial model parameter $\theta_0$. 
% \STATE {\bf Goal:} Find the best model parameter $\theta$ 
% \STATE Initialize $\theta_0$
\FOR{iteration $t$}
    \STATE Randomly sample a labeled batch $\mathcal B_s$ from $\D_s$ and an unlabeled batch 
    $\mathcal B_u$ from $\D_u$.  
    \FOR{each $x$ in $\mathcal B_u$}
    \STATE Apply data augmentation on $x$ for $n$ times, yielding augmented examples $\{x_i'\}_{i=1}^n$
    \STATE {Fixing} $\theta = \theta_{t}$, %{approximate}
    update 
    $\gamma(\cdot|x)$ with %according to \eqref{equ:gammat} as follows,
    \begin{align*}
\gamma_{t+1}(\cdot~|~x) \gets \bigg(  (1-\beta) \times p_{\theta_{t}} (\cdot~|~x)^{1-\alpha} +    \frac{\beta}{n} \times \sum_{i=1}^n  \bigg [ p_{\theta_{t}}(\cdot~|~x_i')^{1-\alpha}\bigg]\bigg )^{\frac{1}{1-\alpha}}.
%\label{equ:empirical_update_gamma}
\end{align*}
     \STATE  Approximate $\Psi_{\alpha, \beta}(\theta, \gamma_{t+1}, x)$ in \eqref{equ:beta_consistency} with augmented examples $\{x_i'\}_{i=1}^n$ accordingly. \vspace{.2\baselineskip}
     \iffalse 
     \begin{align}
\Psi_{\alpha,\beta}(\theta, \gamma_{t+1}, x)  
& \approx (1-\beta )
D_\alpha (\gamma_{t}(\cdot ~|~x) ~\parallel~ p_\theta(\cdot ~|~x) ) %\nonumber 
+ \frac{\beta}{n} \sum_{i=1}^n \Big [ D_\alpha (\gamma_{t}(\cdot ~|~x) ~\parallel~ p_\theta(\cdot ~|~x_i'))   \Big ].
\label{equ:empirical_update_theta}
\end{align}
\fi 
     \ENDFOR
     \STATE  Update $\theta_{t+1}$ by applying one step of gradient descent on \eqref{equ:update_theta} over batch $\mathcal B_u$:
     %\leftarrow \theta_t - \epsilon \Delta \theta$ according to \eqref{equ:update_theta}, with $\epsilon$ the step size, and 
     $$
     %\Delta \theta = 
     \theta_{t+1} \leftarrow \theta_t - \epsilon \nabla_{\theta}\Big(\L(\mathcal B_{s};~ \theta)  + \lambda \E_{x\sim \mathcal B_u}[ \Psi_{\alpha,\beta}(\theta, \gamma_{t+1}, x)]  \Big)
\bigg|_{\theta=\theta_t}.
     $$
     
    % \STATE Update $\theta$ with fixed $\gamma$ with \eqref{equ:update_theta}
    % $$
    % \theta_{t+1} \leftarrow \theta_t - \nabla_\theta  \left [ \L(B_s; \theta) ~+~ \lambda \E_{x\sim B_u, ~ x' \sim \P_x^\beta} \left [D_\alpha (\gamma^*(\cdot~|~x) ~||~ p_\theta(\cdot ~|~ x')) \right]  \right ].
    % $$
    % with $L(\cdot)$ as the supervised loss (e.g. cross entropy). 
\ENDFOR
\end{algorithmic}
\end{algorithm*}


%Note that 
%It is useful to consider special cases. 
%When $\alpha \to 1$, our algorithm can be viewed as a form of EM algorithm. 

%\paragraph{Effect of $\beta$} 


\iffalse 
\paragraph{Effect of $\alpha$} 
The value of $alpha$ plays a critical role in our algorithm. 
The regime of large $\alpha$ ( $\alpha\geq 1$) is of particular interest, and can be seen to resemble FixMatch in a ``soft way''. 
To see this, note that $D_\alpha (\gamma ~||~ p)$ with $\alpha \geq 1$ has a mode covering property, in that when minimizing $p$, a large value of $\gama(y|x)$ implies a large value $p(y|x)$....

To see more, note that the gradient Alpha divergence is
$$
\nabla_\theta 
 D_\alpha(\gamma(\cdot|x)~||~p_\theta (\cdot|x))  
\propto \E_{y\sim \gamma(\cdot | x)}  [w(y|x)\nabla_{\theta} \log p_\theta (y|x) ].
$$
where $w(y|x) = (\gamma(y|x)/p_\theta(y|x))^{\alpha-1}$. 
In comparison, the gradient of FixMatch is similar but with 
$
w(y|x) =(\max_{y} p_{\theta_t}(y|x)) \ind(y = \argmax_y(p_{\theta_t}(y|x))). 
$.... 

%Basically, when 
Overall, when $\alpha$ is large, the significance of large $\gamma(y|x)$ is emphasized when matching $p$, 
and the significance of small $p$ is emphasized when calculating $\gamma$. 
The idea is that $\gamma$ should be determined by the most uncertainty (smallest) part of $p$, while $p$ should be determined by the most confident (largest) part of $\gamma$.  And this achieved by $\alpha \geq 0$. 
\fi 

%We particularly 

% \vspace{-10pt}
% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{tabular}{c}
% \raisebox{1.2em}{\rotatebox{90}{\small  Validation Accuracy}}
% \includegraphics[height=0.23\textwidth]{figures/ablation/beta_curve.pdf}  \\
%  Training epochs ($\alpha=1.5$) \\
% \end{tabular}
% \caption{The Learning curve of AlphaMatch on SVHN, when using  $\alpha=1.5$ and varying $\beta$. 
% %We change the value of $\beta$, using $\alpha=1.5$ and the same labelled data.
% The x-axis denotes the epoch during training and x-axis the validation accuracy. 
% The labelled data includes 4 randomly picked mages per class.
% The dashed line shows the result of FixMatch.
% }
% \label{fig:ablation_beta}
% \vspace{-30pt}
% \end{wrapfigure}

% \paragraph{Impact of $\beta$}


%These additional terms actually have similar impact as some well-studied power divergence, e.g. $\alpha$ / $\beta$ / $\gamma$ divergence.For example, similar to indicator function, the power divergence can also be robust to outliers. We show how different $\alpha$ would impact the gradient and objective.
%\paragraph{$\alpha$ Divergence}
%For $\alpha$ divergence $$D_\alpha(\gamma~||~p)  = \frac{1}{\alpha(\alpha-1)} \left (\E_{\red{p}}\left [\left (\frac{\gamma}{p}\right )^\alpha - 1\right ] \right)$$If $\alpha \to 1$, we have$$\lim_{\alpha \to 1} D_\alpha( \gamma || p) = \E_{p}[\frac{\gamma}{p}\log (\gamma/p)] = \KL( \gamma || p). $$When $\alpha \to 0$, we have $$\lim_{\alpha \to 0} D_\alpha(\gamma || p) =- \E_p [\log (\gamma / p)] = \KL(p || \gamma).$$

%\paragraph{Case Study} We have the gradient of log version $\alpha$ divergence as:$$\nabla_\theta D_\alpha(\gamma || p_\theta)  = \frac{1}{\alpha (\alpha - 1)}\int \frac{\gamma^\alpha}{p_\theta^\alpha} p_\theta \nabla_\theta \log p_\theta(x) = \E_{p_\theta} \left [\left(\frac{\gamma}{p}\right)^\alpha \nabla_\theta \log p_\theta(x) \right ]. $$If $\alpha \to +\infty$, we have $$\nabla_\theta D_\alpha(\gamma || p_\theta)  propto \E_p[ \ind(x = \argmax(\gamma/p)) \nabla_\theta \log p_\theta(x) ] . $$This is more similar to FixMatch \citep{sohn2020fixmatch}, which adds a $\arg\max$ function. 

\paragraph{Time Cost}
% \red{DW. this part is not clear.. }
As shown in Algorithm \ref{alg:main}, our proposed algorithm introduces an additional latent variable $\gamma$ which has a closed-form solution.
Therefore, compared to KL divergence, we introduce almost no additional time cost.




==> semi_supervised_learning _cvpr2021/tex/related_work.tex <==

\section{Related Works}  

% The goal of SSL is to train better prediction models with limited labeled by 
% taking advantage of unlabeled data. 

% \red{modified, take another look}
% \red{a bit repetitive compared to earlier discussions}
Semi-supervised learning (SSL) has been a classical subfield of machine learning with a large literature. 
Examples of classical methods include  
%there is largeliterature on this topic, 
 transductive models \citep[e.g.][]{gammerman2013learning, demiriz1999semi, joachims1999transductive},
 co-training \citep[e.g.][]{blum1998combining,  nigam2000analyzing},  entropy minimization \citep[e.g.][]{grandvalet2005semi, lee2007learning},  graph-based models \citep[e.g.][]{blum2001learning, he2018amc, zhu2002learning, zhou2004learning,  belkin2004regularization, wang2007label, wu2007transductive}
and many more (see \citep[e.g.][]{zhu2005semisurvey, chapelle2009semi}). 
% Earlier works on SSL
% % transdutive models \citep[e.g.][]{gammerman2013learning, }
% % typical consider propagating labels from labeled
% % data to similar unlabeled data 
% % graph-base models \citep[e.g.][]{zhu2005semisurvey, zhu2002learning, zhou2004learning, wang2007label}, 
% % generative modlign? 
% \red{[classical review papers]}. 

Due to the recent success of deep learning,
combining generative model \cite{dai2017good, higgins2016beta} and adversarial training \cite{miyato2015vat} with SSL achieves meaningful improvement over the classic SSL methods in many real-world problems, e.g. image classification \cite{xie2019uda, wang2020attentivenas}, segmentation \cite{papandreou2015weakly}, detection \cite{jeong2019consistency}.
Most recently, data augmentation has been introduced into SSL and achieved great success.
$\Pi$-model, for example,  shares the similar idea of  \eqref{eq:ssl-loss}, but replaces the KL divergence with L2 distance and replace $x$ in \eqref{eq:ssl-loss} with another random copy of augmentation $x''$. 
% VTA, the virtual adversarial training method, replaces the data augmentation method in \eqref{eq:ssl-loss} with an adversarial optimization subject to a neighbouring ball of $x$.
MixMatch \cite{berthelot2019mixmatch} and ReMixMatch \cite{berthelot2019remixmatch}, 
use \emph{mixup} \cite{zhang2017mixup} to do data augmentation.
Based on MixMatch, 
ReMixMatch uses some additional loss and new data augmentation method to improve the performance.
These methods force the label consistency between weakly augmented examples (or examples without augmentation) and strong augmented examples, and improve the state-of-the-art results on classification tasks by a large margin.
% a thread of SSL algorithms have been 
% developed based on combining label consistency with data augmentation, 
% which have been contributing strongly to the recent state-of-the-art performance on strong vision benchmarks.
% Besides UDA, FixMatch, this 
% includes VTA \citep{miyato2015vat}, $\Pi$-Model  \citep{rasmus2015pi},  MixMatch \citep{berthelot2019mixmatch}.  
%Besides UDA and FixMatch that is mostly related work our work, 

Closely related to our work, 
a series of recent SSL methods have been proposed based on the general idea of 
%works rely on 
enforcing the label prediction of an image to be consistent with its augmented counterparts. 
The label consistency has been mostly measured by either KL divergence 
 \citep[e.g.,][]{xie2019uda,berthelot2019mixmatch, berthelot2019remixmatch, miyato2015vat, sohn2020fixmatch}, 
 or mean squared error \citep[e.g.,][]{laine2016temporal, tarvainen2017mean,sajjadi2016regularization,rasmus2015pi}. 
 %And the consistency loss is often minimized 
 Almost all these methods use iterative regularization processes similar to \eqref{eq:ssl-loss}-\eqref{equ:udagrad}, 
 with the stop-gradient trick (see Section \ref{sec:bg}). %, which might suffer from convergence issues. 
%Besides the KL-based methods such as UDA, FixMatch, 
%Typical ways of 
%a line of works uses mean squared error 
%for measuring consistency, 
% including \citet{laine2016temporal, tarvainen2017mean, sajjadi2016regularization},
% or KL divergence, for instance \citet{xie2019uda,berthelot2019mixmatch, berthelot2019remixmatch, miyato2015vat} or hard-thresholding KL divergence, e.g. FixMatch \citep{sohn2020fixmatch}. 
Compared to these works,  
% our alpha-divergence-based measurement offers more flexibility. 
% Furhtermore, 
our method first introduces alpha-divergence as consistency measure,  
and equip it with a convergent EM-like matching algorithm to achieve better results. 
%which offers more flexible in propagating confident-pseudo labels. 
%Meanwhile, our EM-like method has a simple optimization-form, with theoretical convergence guarantees. 
% Meanwhile, our EM-like algorithm enjoys guarantees.  
% EM-like optimization framework with convergence guarantees, allowing us to control the consistency regularization on high confidence instances... 
%in a flexible way by simply varying $\alpha$. 
% to enforce label consistency, or add some extra indicator function, e.g. UDA, FixMatch.
% Although these terms perform well empirically, it may suffer from the convergence problem since the objective does not have a unique solution.
% % what we do
% In this work, we use alpha-divergence as a soft version of these additional terms and further propose an EM-like algorithm to update model parameters, 
% which is also a classic topic for semi-supervised learning \citep[e.g][]{miller1997mixture}.

% The idea of enforcing label consistency was studied extensively in the classical SSL literature; see e.g.,

% Similar ideas of enforcing consistency on augmented data have also attracted wide attention in unsupervised learning; notable examples include \citep{chen2020simclr, he2019moco, wu2018unsupervised, zhuang2019local, oord2018cpc, henaff2019data}.
Most recently, \citet{chen2020exploring} presents a similar EM-like approach for self-supervised learning.
For each step, \citet{chen2020exploring} first closed-form optimizes a local latent variable (similar to our $\gamma$) and then updates the model parameters with a fixed $\gamma$.
This motivates us to further explore our method to more general topics.

%shown 
%Improving consistency has also been shown to be important outside of SSL. 
%Recently, SimCLR \citep{chen2020simclr} proposes to regularize the representations of an image to be similar with each other under label-invariant data augmentation, achieving promising empirical performance in learning effective visual representations. 
%% Similar to this idea, Also, there is a significant body of research along the line of contrastive learning, notable examples include \citep[e.g.][]{he2019moco, wu2018unsupervised, zhuang2019local, oord2018cpc, henaff2019data}.

% \citet{chapelle2009semi} and \citet{zhu2005semisurvey} for reviews.  
% Among all these algorithms, 
% Information regularization principle \citep{chapelle2009semi} and input-dependent  regularization \citep{szummer2003information}, 
% which focus on keeping the label consistency for a set of a priori equivalent examples, 
% are most related.

% Several works improve the performance of SSL 
% via better-desgined data augmentation schemes. 
% % Several works focus on 
% VAT \citep{miyato2015vat} considers enforcing the label predictions to be
% consistent between an image and its corresponding adversarial perturbation  
% within a close neighborhood. 
% MixMatch \citep{berthelot2019mixmatch} show 
% ReMixMatch further improves on MixMatch with 
% CTAugment 

% Earlier works on SSL
% transdutive models \citep[e.g.][]{gammerman2013learning, }
% typical consider propagating labels from labeled
% data to similar unlabeled data 
% graph-base models \citep[e.g.][]{zhu2005semisurvey, zhu2002learning, zhou2004learning, wang2007label}, 
% generative modlign? 


% Alpha-divergence provides a classical tool in probabilistic learning and inference; see e.g., \citep{renyi1961measures, van2014renyi}. 
% Recently, it has been widely studied in approximate inference \citep[e.g.][]{amari2012differential, minka2013expectation, hernandez2016black, li2016renyi, wang2018variational}.   \red{I feel this can be removed}
%\citet{labeau2019experimenting} uses power divergence to learn the representation for rare words in language model.
%\red{alpha-divergence realted work ...}


% Except semi-supervised learning, 
% enforcing label consistency also shows to be helpful in unsupervised learning.
% SimCLR \citep{chen2020simclr}, a recently-proposed unsupervised learning algorithm, 
% replaces $x$ in \eqref{eq:ssl-loss} with another random copy of augmentation $x''$. 
% Other works \citep{he2019moco, wu2018unsupervised, zhuang2019local, oord2018cpc, henaff2019data} do not use data augmentation but force the similarity for data with similar latent representation, 
% which is similar to clustering the data based on their latent representation.
% Some of them also repulse the data belongs to different clusters to be dissimilar.

% Regularizign consistency is useful for self-supervised learning. 
% It also use useful to promote consistency for representation learning.
% Similar ideas have been also investigated for self-supervised learning. 

% Learing by constrating xxx 
% XXX show that incorporating 
% enforcing representations learned for images from different categories to 
% be different with each other 

% \qred{Add SimCLR, MoCo, etc?}%XXXX More.  

